Measurement of the production of a W boson in association with a charm quark in pp collisions at sqrt(s)=7 TeV with the ATLAS detector

The production of a W boson in association with a single charm quark is studied using 4.6 fb^-1 of pp collision data at sqrt(s)=7 TeV collected with the ATLAS detector at the Large Hadron Collider. In events in which a W boson decays to an electron or muon, the charm quark is tagged either by its semileptonic decay to a muon or by the presence of a charmed meson. The integrated and differential cross sections as a function of the pseudorapidity of the lepton from the W-boson decay are measured. Results are compared to the predictions of next-to-leading-order QCD calculations obtained from various parton distribution function parameterisations. The ratio of the strange-to-down sea-quark distributions is determined to be 0.96 +0.26 -0.30 at Q^2=1.9 GeV^2, which supports the hypothesis of an SU(3)-symmetric composition of the light-quark sea. Additionally, the cross-section ratio sigma(W^+ + bar{c})/sigma(W^- + c) is compared to the predictions obtained using parton distribution function parameterisations with different assumptions about the s-bar{s} quark asymmetry.

==> objectselection.tex <==
\section{Event and object selection}
\label{s:objectselection}
Data were collected using either a single-muon
trigger with a requirement on the pseudorapidity of $|\eta^\mu|<2.4$
and on the transverse momentum \ptmu of at least 18\,\GeV\
or a single-electron trigger with pseudorapidity coverage of $|\eta^e|<2.5$
and a minimum threshold on the
transverse energy $E_{\mathrm T}^e$ of 20\,\GeV\ to 22\,\GeV\ depending on the data-taking period.
The algorithms used to select muons and electrons in the trigger are similar
to those used for the offline selection.

Events are required to have at least one primary vertex with at least
three tracks with $\pt > 400\,$\MeV\ reconstructed in the ID.


Further criteria are applied to the tracks used to reconstruct the charm decay products to ensure 
fiducial coverage and good quality. Only tracks with $|\eta|<2.5$ are considered. These tracks are required to have a hit
in the innermost layer of the pixel detector, 
unless the track passes through a region where no hit is expected, and at least 6 SCT hits. 
Only tracks with no more than one missing pixel or SCT hit are used. 
A requirement of $|z_{0}|\sin\theta<15$\,mm (where $z_0$ is the longitudinal impact parameter with respect to the primary vertex and
$\theta$ is the track polar angle)
is applied. No cut on the track impact parameter in the 
transverse plane, $d_0$, is applied to avoid any bias on the selection of tracks coming from a 
displaced \Dsph meson decay vertex. 

$W$ bosons are reconstructed in their leptonic decay channels, 
$W\rightarrow e\nu$ and $W\rightarrow\mu\nu$. Muon candidates are formed from pairs of stand-alone tracks in the ID and the MS that are combined using a $\chi^2$-matching procedure~\cite{atlasmuons,atlasmuonreco}. The charges measured in the ID and the MS are required to be the same. Muons are required to have $\ptmum > 20$\,\GeV.
A cut on the longitudinal impact parameter 
$|z_0|<1$\,mm is applied to remove muons from cosmic-ray background. Tight cuts on the transverse impact parameter significance and the isolation are applied in order to reject muons originating from heavy flavor decays. 
The muon is required to have a transverse impact parameter satisfying $|d_{0}|/\sigma(d_0)<$2.5, where $\sigma(d_0)$ is the uncertainty on the measured $d_0$. 
Both track and calorimeter based isolation requirements are applied: The track-based isolation criterion is defined by requiring the sum of transverse momenta, $\Sigma_{\Delta R < 0.4} \pt^{\rm track}$, of tracks with $\pt^{\rm track}>1\,\GeV$ to be less than 10\% of the muon transverse momentum, where the lepton isolation cone is defined to be $\Delta R = \sqrt{(\phi - \phi_{\ell})^2+(\eta - \eta_{\ell})^2}$. The calorimeter-based isolation is analogously defined as the sum of transverse energies in the calorimeter cells (including electromagnetic and hadronic sections), $\Sigma_{\Delta R < 0.4} E_{\rm T}^{\rm cells}$, and is required to be less than 20\% of \ptmu.

Electrons are selected with transverse momentum \pte$>25$\,\GeV\ and pseudorapidity $|\eta^e|<2.47$, where electrons in the
calorimeter transition region $1.37<|\eta|<1.52$ are excluded. 
To improve the measurement of the electron track parameters, tracks associated 
with the electron are refitted taking into account bremsstrahlung effects using 
a Gaussian Sum Filter (GSF)~\cite{r:gsf}. 
Electrons are required to pass the ``tight'' identification criteria described in Ref.~\cite{Aad:2011mk}, re-optimized for 2011 conditions. In addition, track and calorimeter based 
isolation requirements are applied: $\Sigma_{\Delta R < 0.4} \pt^{\rm track}<\ 0.1\cdot\ptem$ and $\Sigma_{\Delta R < 0.4} E_{\rm T}^{\rm cells}< 0.4\cdot\ptem$. 
The transverse impact parameter significance is required to be $|d_0|/\sigma(d_0)<3$ and the 
longitudinal impact parameter $|z_0|<1$\,mm.

This analysis does not require a reconstructed \Dsp candidate to be associated
with a calorimeter jet. Jets are therefore used only as input to the calculation of missing 
transverse energy (\met) and to reject background from top-quark pair production. Jets are reconstructed using the
infrared- and collinear-safe anti-$k_t$ algorithm~\cite{bib:antikt2}
with radius parameter $R=0.4$
using the FastJet package~\cite{bib:antikt3}.
The detector input is based on topological clusters~\cite{bib:topo}.
Jets are calibrated using the EM+JES scheme~\cite{Aad:2011he}.

The magnitude and azimuthal direction of \met\ are measured from the vector sum of the transverse
momentum of calibrated physics objects~\cite{r:MetPerf}. 

To reduce the dominant multi-jet background,  the \met\ is required to be greater than 25\,\GeV\ in the $W$ selection and the transverse mass, \mtw\, of the $W$ boson is required to be greater than 40\,\GeV. The transverse mass, \mtw, is defined as $\mtw \equiv \sqrt{2p_T^l\met(1-\rm{cos}\Delta\phi)}$, where $\Delta\phi$ is the azimuthal separation 
between the directions of the lepton and the missing energy in the transverse plane.

Events with an additional electron or muon are vetoed to suppress background from $Z$ and $t\overline{t}$ 
events. For this veto, a looser lepton selection is applied: the \pt\ cut on the electron is 
lowered to 20\,\GeV, the electron identification criteria are relaxed to ``medium''~\cite{Aad:2011mk} (re-optimized for 2011 conditions) and electrons and 
muons are not required to pass the impact parameter and isolation requirements. 
In order to suppress background from $t\overline{t}$ events, 
events with 3 or more jets with $\pt>25$\,\GeV\ and $|\eta|<2.5$ are rejected. 


